NormMark: A Weakly Supervised Markov Model for Socio-cultural Norm Discovery

Norms, which are culturally accepted guidelines for behaviours, can be integrated into conversational models to generate utterances that are appropriate for the socio-cultural context. Existing methods for norm recognition tend to focus only on surface-level features of dialogues and do not take into account the interactions within a conversation. To address this issue, we propose NormMark, a probabilistic generative Markov model to carry the latent features throughout a dialogue. These features are captured by discrete and continuous latent variables conditioned on the conversation history, and improve the model's ability in norm recognition. The model is trainable on weakly annotated data using the variational technique. On a dataset with limited norm annotations, we show that our approach achieves higher F1 score, outperforming current state-of-the-art methods, including GPT3.

==> sections/03_method.tex <==
\section{Hidden semi-Markov Model for Socio-cultural Norm Discovery}

Given a set of dialogues $\mathcal{D} = \{d^1, \dots, d^n\}$, where each dialogue consists of a set of segments $d^i = \{ s_1^i, \dots, s_m^i\}$ in which each segment consists of a \sout{set} \yf{sequence} of tokens from vocabulary set $\mathcal{V}$. The dialogue set $\mathcal{D}$ consists of two subsets of observed~($\mathcal{D}_O$) and unobserved~($\mathcal{D}_U$) dialogues, where each segment $s_m^i \in \mathcal{D}_O$ corresponds to a socio-cultural norm label $c \in \mathcal{C} = \{c_k\}_{k=1}^K$. Segments $s_m^i \in \mathcal{D}_U$ lack socio-cultural norm labels. Our goal is to develop a model that, by using contextual information carried from previous segments of the dialogue, discovers the socio-cultural norm associated with a segment of a given dialogue.

To this end, we introduce a segment-level latent variable $z$ that captures contextual representation of each segment. We assume a Hidden semi-Markov Model~(HSMM) that models the joint probability of the labels and segments as follows:

\begin{align}
    P_{\theta}(\overrightarrow{s}_1, \dots ,\overrightarrow{s}_T,\{c_{i}\}_{\mathcolorbox{i \in O}}) &= \\ \nonumber
    \int_{z_1}\dots \int_{z_T} \sum_{c_{j_1}}\dots \sum_{c_{\mathcolorbox{j_{|U|}}}} & \\ \nonumber
    P(\overrightarrow{s_1}, \overrightarrow{z_1}, c_1, \dots, \overrightarrow{s_t}, \overrightarrow{z_t}, c_t) d_{\overrightarrow{z_1}} \dots d_{\overrightarrow{z_T}}
\end{align}
\yf{some notations above (e.g. $O$ and $U$) are undefined. Need to go over and revise}
which can be further factorised into:
\begin{align}
    P_{\theta}&(\overrightarrow{s_1}, \overrightarrow{z_1}, c_1, \dots, \overrightarrow{s_t}, \overrightarrow{z_t}, c_t) = \\ \nonumber
    \prod_{t=1}^{T} &P_{\theta}(c_t | c_{t-1}, \overrightarrow{s_t}).P_{\theta}(\overrightarrow{z_t}|\overrightarrow{z_{t-1}}, \overrightarrow{s_t}).P_{\theta}(\overrightarrow{s_{t}}|c_{t},\overrightarrow{z_{t}})
\end{align}
where $\theta$ denotes the parameters of our model. 

To learn a semi-supervised Variational Autoencoder~(VAE) based on the above graphical model, we optimise the variational lower band. 

For unlabelled data:
\begin{align}
    \mathcal{L}_U~&(\overrightarrow{s})  = \log\ p(\overrightarrow{s}) \geq \\
    &\mathbb{E}_{q(c|\overrightarrow{s},c_{t-1})}[\mathbb{E}_{\overrightarrow{z}\sim q(\overrightarrow{z}|\overrightarrow{s},\overrightarrow{z_{t-1}})} 
    [\log p(\overrightarrow{s}|\overrightarrow{z},c)] \nonumber \\
    &- \bm{KL}[q(\overrightarrow{z}|\overrightarrow{s}, \overrightarrow{z_{t-1}})||p(\overrightarrow{z})]] \nonumber \\
    & -\bm{KL}[q(c|\overrightarrow{s}, c_{t-1})||p(c)] \nonumber
\end{align}
where $q(c|\overrightarrow{s}, c_{t-1})$ is a classification network~(including an encoder) for predicting segment-level labels, and $p(\overrightarrow{s}| \overrightarrow{z},c)$ is a decoder. 

For labelled data:
\begin{align}
    \mathcal{L}_O~&(\overrightarrow{s}, c) = \log p(\overrightarrow{s}, c) \geq \\
    &\mathbb{E}_{\overrightarrow{z} \sim q(\overrightarrow{z}|\overrightarrow{s}, \overrightarrow{z_{t-1}})}[\log p(\overrightarrow{s}|\overrightarrow{z},c)] \nonumber \\ 
    &- \bm{KL}[q(\overrightarrow{z}|\overrightarrow{s},\overrightarrow{z_{t-1}})||p(\overrightarrow{z})] + constant \nonumber
\end{align}
where the parameters of the classification network $q(c|\overrightarrow{s}, c_{t-1})$ are updated by minimising the cross entropy loss $\mathbb{E}_{(\overrightarrow{s},c)}[-\log q(c|\overrightarrow{s})]$, directly.

The overall loss function of our proposed approach then is:

\begin{equation}
    \mathcal{L} = \mathbb{E}_{s \in \mathcal{D}_U}\mathcal{L}_U~(\overrightarrow{s}) + \lambda \mathbb{E}_{s \in D_{O}}\mathcal{L}_O~(\overrightarrow{s}, c)
\end{equation}
where $\lambda$ controls the trade-off between the classifier network's loss and the generative loss.

==> tables/01.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l    c  c  c  c  c  c  c  c  c}
            & \multicolumn{3}{c}{\textbf{50}} & \multicolumn{3}{c}{\textbf{100}} & \multicolumn{3}{c}{\textbf{Max}} \\
            \toprule[0.1em]
            \textbf{Model} &  \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} & \textbf{P} & \textbf{R} & \textbf{F1} \\
            \toprule[0.1em]
            LSTM &  7.92 & 12.5 & 9.69 & 11.06 & 12.58 & 9.90 & 9.13 & 12.57 & 10.08 \\
            BERT &  10.85 & 15.74 & 12.58 & 10.46 & 15.50 & 11.82 & 38.42 & 32.33 & 33.34 \\
            WS-VAE-BERT &  20.43 & 17.21 & 16.60 & 36.38 & 22.48 & 23.37 & 42.03 & \textbf{40.74} & 39.01 \\
            SetFit & 30.42 & 26.25 & 27.86 & 32.12 & 30.54 & 31.32 & 41.42 & 40.23 & 40.54 \\
            %NormBank & P & R & F1 & P & R & F1 & P & R & F1 & P & R & F1 \\
            \hline
            GPT-3 &  \textbf{39.86} & \textbf{35.05} & \textbf{33.61} & \textbf{39.86} & \textbf{35.05} & 33.61 & 39.86 & 35.05 & 33.61 \\
            \hline
            $\textsc{NormMark}_{\texttt{zero}}$ &  25.94 & 19.71 & 20.04 & 35.41 & 27.73 & 28.33 & 44.14 & 36.97 & 39.49 \\
            \textsc{NormMark} &  \textbf{32.46} & \textbf{30.02} & \textbf{30.72} & \textbf{36.41} & \textbf{33.48} & \textbf{34.43} & \textbf{47.92} & 38.67 & \textbf{44.20} \\
            \toprule[0.1em]
    \end{tabular}}
    \caption{Segment-level socio-cultural norm prediction performance~(precision, recall and F1 score). The results are reported by training the models on 50, 100, and maximum number of labelled sequences of dialogues.}
    \label{tab:main-results}
    %\vspace{-2ex}
\end{table*}





==> tables/05_graphical_model_extended.tex <==
\begin{figure}[t]
	   \centering
	   \includegraphics[width=0.5\textwidth]{figs/Norm Mark Extended - Aligned.pdf}
\caption{The graphical representation of two extended variation of $\textsc{NormMark}$ and $\textsc{NormMark}_\texttt{zero}$.}
\label{fig:g-model}
\end{figure}
